DAS: A Deformable Attention to Capture Salient Information in CNNs

Convolutional Neural Networks (CNNs) excel in local spatial pattern recognition. For many vision tasks, such as object recognition and segmentation, salient information is also present outside CNN's kernel boundaries. However, CNNs struggle in capturing such relevant information due to their confined receptive fields. Self-attention can improve a model's access to global information but increases computational overhead. We present a fast and simple fully convolutional method called DAS that helps focus attention on relevant information. It uses deformable convolutions for the location of pertinent image regions and separable convolutions for efficiency. DAS plugs into existing CNNs and propagates relevant information using a gating mechanism. Compared to the O(n^2) computational complexity of transformer-style attention, DAS is O(n). Our claim is that DAS's ability to pay increased attention to relevant features results in performance improvements when added to popular CNNs for Image Classification and Object Detection. For example, DAS yields an improvement on Stanford Dogs (4.47%), ImageNet (1.91%), and COCO AP (3.3%) with base ResNet50 backbone. This outperforms other CNN attention mechanisms while using similar or less FLOPs. Our code will be publicly available.

==> sections/ablation.tex <==
\subsection{Ablation Study}\label{sec:ablation}

Before zeroing in on the design of DAS attention gate, we tested various pixel-wise attention ideas. Two of them which led us to the current design are as follows.

Idea \#1: First we concatenated the input with a GridSample of it and then fed it to another convolution layer which combined the input and the learned far pixels. GridSample is an operation that takes an input tensor and a grid tensor, and it computes the spatial interpolation of nearhood pixels.

Formulas:

$output = GridSample(x)$

$output = concatenation(x, output)$

$output = conv(output)$


Idea \#2: It is similar to the first idea but uses the compressed inputs and GridSample outputs and calculates weights between 0 and 1 to suppress the additional information in the features.

Formulas:

$compressed\_input = conv1(x)$

$Compressed\_gridsample = GridSample(conv2(x))$

$output = concatenation(compressed\_input, Compressed\_gridsample)$

$output = conv3(output)$

$output = torch.mul(x, output)$

\begin{table}[]
\begin{tabular}{cccc}
\multicolumn{1}{l}{Idea} & \multicolumn{1}{l}{Accuracy(Dogs)} & \multicolumn{1}{l}{FLOPs (B)} & Parameters (M) \\
Idea \#1                 & 65                                  & 1.99                         & 12.766            \\
Idea \#2                 & 65.21                               & 1.846                         & 11.801          \\
Current method           & \textbf{66.41}                      & 1.856                         & 11.817          
\end{tabular}
\end{table}


To show that every part of the method is positively cooperating in the performance of the attention method, we conducted experiments on all parts of the proposed gate. For the first experiment, we deleted the first part of the method and only used the deformable convolution to calculate attention weights. Since the bottleneck was removed, the flops and number of parameters were increased but the accuracy was also decreased. Which shows the importance of the first convolution layer.

In the next experiment, by removing deformable convolution and keeping the first part, the attention module will only have one convolutional layer that provides the attention weights. The results show that this decreased accuracy.
Further, to see whether the deformable convolutional layer really helps, we changed the deformable conv with a regular conv layer. Although it slightly decreased FLOPs and number of parameters, the accuracy also decreased. This experiment clearly shows that the deformable convolutional layer does indeed enable focusing attention to salient features better than a regular conv layer.

\begin{table}[]
\begin{tabular}{cccc}
\multicolumn{1}{l}{Models for ablation study} & \multicolumn{1}{l}{Accuracy (Dogs)} & \multicolumn{1}{l}{FLOPs (B)} & Parameters (M) \\
1 Conv. layer                                 & 65.338                              & 1.915                               & 11.923               \\
1 Depthwise Sep. Conv.                        & 65.291                              & 1.879                               & 12.048               \\
2 Depthwise Sep. Conv.                        & 66.107                              & 1.849                               & 11.843               \\
GS18                                          & \textbf{66.41}                      & 1.856                               & 11.817              
\end{tabular}
\end{table}

In another experiment, the effect of alpha was studied. As alpha increases from 0 to 1, flops and number of parameters increase. The results show that alpha more than 0.1 has decent results. In most cases, there is a trade off between flops and accuracy, so we chose alpha=0.2 for our experiments.

\begin{table}[]
\begin{tabular}{cccc}
\multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Alpha\\ (ablation study)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Accuracy\\ (Dogs)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}FLOPs\\ (B)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Parameters\\ (M)\end{tabular} \\
$\alpha$= 0.01                                                                         & 65.315                                                                        & 1.829                                                                   & 11.706                                                   \\
$\alpha$= 0.1                                                                          & 66.224                                                                        & 1.842                                                                   & 11.759                                                   \\
\begin{tabular}[c]{@{}c@{}}alpha = 0.2\\ (current)\end{tabular}                      & \textbf{66.41}                                                                & 1.856                                                                   & 11.817                                                   \\
$\alpha$= 0.3                                                                          & 65.944                                                                        & 1.871                                                                   & 11.875                                                   \\
$\alpha$= 0.4                                                                          & 65.956                                                                        & 1.885                                                                   & 11.933                                                   \\
$\alpha$= 0.5                                                                          & \textbf{66.527}                                                               & 1.899                                                                   & 11.99                                                    \\
$\alpha$= 1                                                                            & \textbf{66.83}                                                                & 1.97                                                                    & 12.282                                                  
\end{tabular}
\end{table}



Furthermore, to investigate the effect of numbers of attention layers, we added attention layers after all skip connections. Although it improves the performance slightly, FLOPS and parameters are also increased, especially in larger models. So we concluded that four attention layers are good with regard to computation cost and its accuracy. Other studies have been done and the final proposed attention model was chosen by care to be simple, efficient and accurate on both small and large datasets.

\begin{table}[]
\begin{tabular}{clcc}
\multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Effect of \# layers\\ (ablation study)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Accuracy\\ (Dogs)\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}FLOPs\\ (B)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Parameters\\ (M)\end{tabular} \\
\begin{tabular}[c]{@{}c@{}}GS18\_all\_layers\\ (TEST 300)\end{tabular}                             & \multicolumn{1}{c}{66.783}                                & 1.889                                                                   & 11.944                                                   \\
\begin{tabular}[c]{@{}c@{}}GS18\_4\_layers\\ (current)\end{tabular}        & \multicolumn{1}{c}{66.41}                                 & 1.856                                                                   & 11.817                                                   \\
GS50\_all\_layers                                                                                  & \textbf{}                                                 & 5.115                                                                   & 30.477                                                   \\
\begin{tabular}[c]{@{}c@{}}GS50\_4\_layers\\ (current)\end{tabular}                                &                                                           & 4.387                                                                   & 26.899                                                  
\end{tabular}
\end{table}

